Train Where the Data is: A Case for Bandwidth Efficient Coded Training

Training a machine learning model is both compute and data-intensive. Most of the model training is performed on high performance compute nodes and the training data is stored near these nodes for faster training. But there is a growing interest in enabling training near the data. For instance, mobile devices are rich sources of training data. It may not be feasible to consolidate the data from mobile devices into a cloud service, due to bandwidth and data privacy reasons. Training at mobile devices is however fraught with challenges. First mobile devices may join or leave the distributed setting, either voluntarily or due to environmental uncertainties, such as lack of power. Tolerating uncertainties is critical to the success of distributed mobile training. One proactive approach to tolerate computational uncertainty is to store data in a coded format and perform training on coded data. Encoding data is a challenging task since erasure codes require multiple devices to exchange their data to create a coded data partition, which places a significant bandwidth constraint. Furthermore, coded computing traditionally relied on a central node to encode and distribute data to all the worker nodes, which is not practical in a distributed mobile setting. In this paper, we tackle the uncertainty in distributed mobile training using a bandwidth-efficient encoding strategy. We use a Random Linear Network coding (RLNC) which reduces the need to exchange data partitions across all participating mobile devices, while at the same time preserving the property of coded computing to tolerate uncertainties. We implement gradient descent for logistic regression and SVM to evaluate the effectiveness of our mobile training framework. We demonstrate a 50% reduction in total required communication bandwidth compared to MDS coded computation, one of the popular erasure codes.

==> 0.smaller_abstract.tex <==
Training a machine learning model is both compute and data-intensive. Most of the model training is performed on high performance compute nodes and the training data is stored near these nodes for faster training. But there is a growing interest in enabling training near the data. For instance, mobile devices are rich sources of training data. It may not be feasible to consolidate the data from mobile devices into a cloud service, due to bandwidth and data privacy reasons. Training at mobile devices is however fraught with challenges. First mobile devices may join or leave the distributed setting, either voluntarily or due to environmental uncertainties, such as lack of power. Tolerating uncertainties is critical to the success of distributed mobile training. One proactive approach to tolerate computational uncertainty is to store data in a coded format and perform training on coded data. Encoding data is a challenging task since erasure codes require multiple devices to exchange their data to create a coded data partition, which places a significant bandwidth constraint. Furthermore, coded computing traditionally relied on a central node to encode and distribute data to all the worker nodes, which is not practical in a distributed mobile setting.

In this paper, we tackle the uncertainty in distributed mobile training using a bandwidth-efficient encoding strategy. We use a Random Linear Network coding (RLNC) which reduces the need to exchange data partitions across all participating mobile devices, while at the same time preserving the property of coded computing to tolerate uncertainties. We implement gradient descent for logistic regression and SVM to evaluate the effectiveness of our mobile training framework. We demonstrate a 50% reduction in total required communication bandwidth compared to MDS coded computation, one of the popular erasure codes.

==> 5.old.implementation.tex <==
In this section we briefly describe the applications that we evaluated. %Since matrix-vector multiplication forms the heart of many training algorithms, we first focus on it in our implementation. Then we will describe the implementation details of our mobile coded computation framework.

\subsection{Computing Applications}
Gradient descent is popularly used for training machine learning and deep learning models. It is an iterative optimization algorithm which uses matrix-vector multiplication during each iteration. So we evaluated our proposed \emph{mobile training framework} on two machine learning algorithms: Logistic Regression and Support Vector Machine (SVM). Next we describe their implementations in our system.
\subsubsection{Logistic Regression}\label{LRSection}
Logistic regression is a machine learning algorithm widely used to do binary classification. It uses a sigmoid function $ \sigma(a) = \frac{1}{1+e^{(-a)}}$ to classify.
%We implemented a distributed synchronous gradient descent algorithm to minimize the cross-entropy error function.
In general, gradient descent has the following form: if \(\boldsymbol{w}\) is the parameter of interest, \(\eta\) is the learning rate, \(\lambda\) is the regularization coefficient, \(\boldsymbol{t}\) is the iteration variable: \(\boldsymbol{w}^{(t+1)} = \boldsymbol{w}^{(t)} - \eta (\nabla \boldsymbol{w}^{(t)} + \lambda\boldsymbol{w})\). 
For logistic regression where we have \(\boldsymbol{X}\) as the matrix representing all the training features and \(\boldsymbol{y}\) as the vector representing training class labels, the gradient can be written as: \(\nabla \boldsymbol{w}^{(t)} = \boldsymbol{X}^{T} 
(\sigma(\boldsymbol{X}\boldsymbol{w}^{(t)})-\boldsymbol{y})\). 

We can observe that there are two major matrix-vector multiplications, \(\boldsymbol{X}\boldsymbol{w}^{(t)}\) and \(\boldsymbol{X}^{T} \boldsymbol{p}\) where \(\boldsymbol{p} = \sigma(\boldsymbol{X}\boldsymbol{w}^{(t)})-\boldsymbol{y}\).
%The gradient descent procedure implemented in our system for Logistic Regression is described in Algorithm \ref{alg:LR}. 
During each iteration of Gradient Descent these two matrix-vector products are used to calculate the gradient of the weight vector. In our framework, the two matrix-vector multiplications are coded and parallelized by computing partial matrix-vector products at different workers and then constructing the total matrix-vector product at the end of each iteration.

\begin{comment}
%COMMENTED FOR SYSML SPACE
\begin{algorithm}
\caption{Gradient Descent for Logistic Regression}
\label{alg:LR}
\begin{algorithmic}
\State \textbf{Input:} Dataset $D(i)$ for $i = 1$ to $K$ that are stored distributedly in $K$ workers, $(N,K)$ Coding Strategy $Coding$, Number of iterations $numIter$
\State \textbf{Output:} weight vector of the trained model $w$
\State Preprocess the dataset $D(i)$ and generate sub matrix $X(i)$, $X^{T}(i)$ for $i = 1$ to $K$ and class labels $y$
\State Encode $X(j)$, $X^{T}(j)$ as per $Coding$ for $j = K+1$ to $N$ distributedly at the remaining $(N-K)$ workers 
\State Initialize vector $w$ to random values
%\State $iter \leftarrow 0$
\For {$iter$ = 0 to $numIter$}
    \State compute \(\boldsymbol{X}\boldsymbol{w}^{(t)}\) by performing coded computation 
    \State p = $\sigma(\boldsymbol{X}\boldsymbol{w}^{(t)})-\boldsymbol{y}$
    \State compute $\nabla \boldsymbol{w}^{(t)} = \boldsymbol{X}^{T} \boldsymbol{p}$ by performing coded computation 
    \State  $\boldsymbol{w}^{(t+1)} = \boldsymbol{w}^{(t)} - \eta (\nabla \boldsymbol{w}^{(t)} + \lambda\boldsymbol{w})$
    \State $iter \leftarrow iter + 1$
\EndFor
\State return $w$
\end{algorithmic}
\end{algorithm}

\end{comment}

\subsubsection{SVM}
Support Vector Machine (SVM) is another commonly used supervised learning model for binary classification of data. For SVM where we have \(\boldsymbol{X}\) as the matrix representing training features and \(\boldsymbol{y}\) as the vector representing training labels, the model can be represented as: \(\boldsymbol{s} = \boldsymbol{X}\boldsymbol{w}^{(t)}\). By considering N as the total number of samples in training data, the sub-gradient can be expressed as: \(\nabla \boldsymbol{w}^{(t)} = \frac{1}{N}\boldsymbol{X}^{T} \boldsymbol{m}\), where m is a vector with \(\boldsymbol{m}_j = -\boldsymbol{y}_j \text{ if \(\boldsymbol{y}_j\boldsymbol{s}_j < 1\) otherwise 0}\).
We can observe that there are two major matrix-vector multiplications here, \(\boldsymbol{X}\boldsymbol{w}^{(t)}\) and \(\boldsymbol{X}^{T} \boldsymbol{m}\). These matrix-vector multiplications are parallelized by computing partial matrix-vector products at different workers and then constructing the total matrix-vector product at the master as described in Algorithm \ref{alg:SVM}. 

\begin{algorithm}[H]
\caption{Gradient Descent for SVM}
\label{alg:SVM}
\begin{algorithmic}
\State \textbf{Input:} Dataset $D(i)$ for $i = 1$ to $K$ that are stored distributedly in $K$ workers, $(N,K)$ Coding Strategy $Coding$, Number of iterations $numIter$
\State \textbf{Output:} weight vector of the trained model $w$
\State Preprocess the dataset $D(i)$ and generate sub matrix $X(i)$, $X^{T}(i)$ for $i = 1$ to $K$ and class labels $y$
\State Encode $X(j)$, $X^{T}(j)$ as per $Coding$ for $j = K+1$ to $N$ distributedly at the remaining $(N-K)$ workers 
\State Initialize vector $w$ to random values
%\State $iter \leftarrow 0$
\For {$iter$ = 0 to $numIter$}
    \State compute \(\boldsymbol{X}\boldsymbol{w}^{(t)}\) by performing coded computation
    \State compute $m$
    \State compute $\nabla \boldsymbol{w}^{(t)} =\boldsymbol{X}^{T} \boldsymbol{m}$ by performing coded computation
    \State  $\boldsymbol{w}^{(t+1)} = \boldsymbol{w}^{(t)} - \eta (\nabla \boldsymbol{w}^{(t)} + \lambda\boldsymbol{w})$
    \State $iter \leftarrow iter + 1$
\EndFor
\State return $w$
\end{algorithmic}
\end{algorithm}

\subsection{System Setup}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/rpis.png}
    \caption{Picture of our Edge Cluster}
    %\vspace{-3cm}
    \label{fig:rpis}
\end{figure}
We evaluated the above computing applications on a Raspberry Pi cluster, which mimics a representative edge computing environment. This cluster is composed of 22 identical Raspberry Pi 3 Model B nodes. Each node consists of a Quad Core 1.2GHz Broadcom BCM2837 64bit CPU, running HypriotOS V1.7.0 with Linux Kernel 4.4.50. Each Raspberry Pi has 1GB of DRAM and a 64G Western Digital PiDrive connected through USB. And all of the 22 nodes are connected under a wireless network. We bootstrap this Raspberry Pi cluster with Kubernetes and we dockerize our computing applications to run on the Kubernetes cluster. Figure \ref{fig:rpis} is a picture of our Raspberry Pi cluster system. With this setup, we can also expand our cluster with more Raspberry Pi nodes and scale up the existing applications and deploy them on the cluster easily. %We implemented our framework using python and bash scripts.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth, height=6.5cm]{plots/flowChart.png}
    \caption{Phases in Edge Coded Computation}
    %\vspace{-3cm}
    \label{fig:phases}
\end{figure}
\subsection{Implementation details}
Now we describe the workings of our edge coded computation framework, which is shown in figure \ref{fig:phases}. 22 docker containers are launched onto the Raspberry Pi cluster, representing the workers of the computation task. Each of these worker docker containers is running on a separate Raspberry Pi node. Another docker container is launched within the same cluster to represent the master. Unlike in~\cite{speedUpML} where the master needs to encode and distribute the coded sub-matrices to the workers, our master docker container is simply responsible for coordinating the workers and decoding the matrix-vector multiplication product at the end of each iteration. Since the master docker container is a lightweight coordinator and decoder, it can easily coexist with any of the worker docker containers on the same Raspberry Pi node. 

At the beginning of computation, master sends the $(N, K)$ generator matrix $G$ to each of the workers. While the first $K$ workers have original sub-matrix and do not require encoding, the remaining $(N-K)$ workers request and download their needed sub-matrices from the first $K$ workers to perform encoding based on the generator matrix $G$. Due to the highly constrained memory space, the remaining $(N-K)$ workers need to load the sub-matrices one by one to do the encoding once they obtain their needed copies. 

One iteration of our \emph{edge coded computation} is described in \ref{alg:codedComputing}. At the start of each iteration of our applications, the master distributes the vector to be multiplied to all workers and informs the workers to start their computation tasks. At the end of each iteration, master receives the sub-products from the workers, decodes them and constructs the result vector. Each worker has two separate running processes, one for computation and one for communication. The computation process on the worker is straightforward. During each iteration it simply multiplies the sub-matrix with the vector received from the master, generates the partial product and then waits for the next iteration of computation. The communication process is in charge of receiving input data from the master, sending the partial product, and controlling the start and stop of the computation process at the worker.  

\begin{algorithm}[H]
\caption{One iteration for edge coded computation}
\label{alg:codedComputing}
\begin{algorithmic}
\State Master broadcast $V$ to all workers at the beginning of an iteration
%\State $iter \leftarrow 0$
\State $set \leftarrow \phi$
\State $partialP_{dict} \leftarrow \phi$
\While {$set$ is not decodable}
    \State \textbf{on} Receiving completion of partial product $p$ computation message from worker $w$
    \State $set \leftarrow (set, w)$
    \State $partialP_{dict} \leftarrow (partialP_{dict}, p_{w})$
\EndWhile
\State Cancel computation at the remaining stragglers
\State $P \leftarrow decode(set, partialP_{dict})$
\end{algorithmic}
\end{algorithm}

%%%%
